PARTNR: A Benchmark for Planning and Reasoning in Embodied Multi-agent Tasks

We present a benchmark for Planning And Reasoning Tasks in humaN-Robot collaboration (PARTNR) designed to study human-robot coordination in household activities. PARTNR tasks exhibit characteristics of everyday tasks, such as spatial, temporal, and heterogeneous agent capability constraints. We employ a semi-automated task generation pipeline using Large Language Models (LLMs), incorporating simulation in the loop for grounding and verification. PARTNR stands as the largest benchmark of its kind, comprising 100,000 natural language tasks, spanning 60 houses and 5,819 unique objects. We analyze state-of-the-art LLMs on PARTNR tasks, across the axes of planning, perception and skill execution. The analysis reveals significant limitations in SoTA models, such as poor coordination and failures in task tracking and recovery from errors. When LLMs are paired with real humans, they require 1.5x as many steps as two humans collaborating and 1.1x more steps than a single human, underscoring the potential for improvement in these models. We further show that fine-tuning smaller LLMs with planning data can achieve performance on par with models 9 times larger, while being 8.6x faster at inference. Overall, PARTNR highlights significant challenges facing collaborative embodied agents and aims to drive research in this direction.

==> 01_abstract.tex <==
\begin{abstract}
We present a benchmark for Planning And Reasoning Tasks in humaN-Robot collaboration (\bench{}) designed to study human-robot coordination in household activities. \bench{} tasks exhibit characteristics of everyday tasks, such as spatial, temporal, and heterogeneous agent capability constraints. We employ a semi-automated task generation pipeline using Large Language Models (LLMs), incorporating simulation-in-the-loop for the grounding and verification. \bench{} stands as the largest benchmark of its kind, comprising 100,000 natural language tasks, spanning 60 houses and 5,819 unique objects. We analyze state-of-the-art LLMs on \bench{} tasks, across the axes of planning, perception and skill execution. The analysis reveals significant limitations in SoTA models, such as poor coordination and failures in task tracking and recovery from errors. When LLMs are paired with \emph{real} humans, they require 1.5$\textsc{x}$ as many steps as two humans collaborating and 1.1$\textsc{x}$ more steps than a single human, underscoring the potential for improvement in these models. We further show that fine-tuning smaller LLMs with planning data can achieve performance on par with models 9 times larger, while being 8.6$\textsc{x}$ faster at inference. Overall, \bench{} highlights significant challenges facing collaborative embodied agents and aims to drive research in this direction. 
\end{abstract}


==> figs/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> prompts/multi_agent_react_summary_fo.tex <==
\begin{mdframed}[
    linewidth=1pt, % Width of the border line
    linecolor=black, % Color of the border line
    backgroundcolor=gray!10, % Background color of the box
    roundcorner=5pt, % Round cornered box
    frametitle={Multi Agent | ReAct-Summary | Decentralized | Full Observability},
    frametitlealignment=\center % Center align the frame title
]

\begin{prompt}
<|start_header_id|>system<|end_header_id|>
- Overview:
Your goal is to find the optimal next action for an agent collaborating with another agent in a multi-agent planning task. Find action for the agent as best as you can. The task assigned to you will be situated in a house and will generally involve navigating to objects, picking and placing them on different receptacles to achieve rearrangement. Below is the detailed description of different actions that the agent can use for solving the task. You can assign them to Agent_{id} as required. Remember to assign only 1 action to your agent. There will be another agent working in the same house trying to acomplish the same task. Your role is to enable Agent_{id} to finish the task together by collaborating with its partner agent.

You should account for the task progress, locations of objects in the house, the partner agent's previous and current actions, and your agent's observations to determine the next optimal action for your agent. The optimal action should be aimed at enabling faster and more efficient task completion. So avoid doing tasks that the partner agent is doing and instead focus on tasks that are left over and can be done in parallel. You should also evaluate task progress and exit the task with a final thought if the task requirements are already satisfied.

{tool_descriptions}
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Here are some examples of allocating optimal next actions to the agents in a given task:

Example 1:
Task:
Move all objects from sofa to bedroom and place them next to the toy truck.

House description:
living_room_0: chair_0, chair_1, chair_2, chair_3, table_0, couch_0, couch_1, table_1, table_2, table_3
closet_0: shelves_0
bedroom_0: bed_0, chest_of_drawers_0, chest_of_drawers_1
kitchen_1: cabinet_0, table_4, chair_4, chair_5, chair_6, chair_7
bedroom_1: bed_1, chest_of_drawers_2, chest_of_drawers_3
bedroom_2: bed_2, chest_of_drawers_4, chest_of_drawers_5, wardrobe_0, wardrobe_1
laundryroom/mudroom_0: washer_dryer_0, washer_dryer_1, shelves_1, shelves_2
bathroom_0: toilet_0
bathroom_2: toilet_1
bathroom_1: toilet_2
kitchen_0: fridge_0
garage_0: fridge_1

Objects in the house:
cherry_0: couch_0
apple_0: agent_1
banana_0: couch_0
toy_fire_truck_0: bed_1

Task progress:
Agent 0 is walking somewhere.
Agent 1 is moving with apple_0 to rearrange it.

Your agent's observations of the last executed action (if available):
Agent_0_observation: Unexpected failure! - Failed to pick! This object is with another agent.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Based on the task and the list of objects in the house, the current task-relevant objects are cherry_0, banana_0, apple_0 located on the couch_0, couch_0, and agent_1 respectively. The desired location for these objects is on the bed, specifically next to the toy truck based on the task description. So I will choose the bed where toy truck is located as target location for these objects. I will use the exact name of the bed provided in house description. Based on the object locations provided in the object list and the task progress summary, Agent 1 is currently rearranging apple_0. Agent 0's previous action execution failed because Agent 1 was already rearranging that object. So I will ask my Agent 0 to rearrange one of the other task-relevant objects cherry_0 or banana_0.
Agent_0_Action: Rearrange[cherry_0, on, bed_1, next_to, toy_fire_truck_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Example 2:
Task:
Move pillows to bed and then move apple to kitchen counter.

House description:
living_room_0: table_0, couch_0, chair_2, shelves_1, chair_5, chair_6, table_7, chair_7, chair_8, chair_9, chair_10, chair_11, chair_12, table_9, table_10, stand_0, chest_of_drawers_2
laundryroom/mudroom_0: washer_dryer_0, washer_dryer_1, shelves_0
bathroom_1: bathtub_0, table_11
bedroom_1: table_1, chair_1, bed_0, table_4, table_5, chair_4, stool_0, bench_0, table_12, chest_of_drawers_3
kitchen_0: cabinet_0, cabinet_1, cabinet_2, counter_0, chair_2, cabinet_3, cabinet_4, cabinet_5, chair_13, chair_14, chair_15, counter_1, cabinet_6, fridge_0, cabinet_7, cabinet_8
bedroom_0: chair_0, table_2, table_3, bed_1, bench_2, chest_of_drawers_0, chest_of_drawers_1
bathroom_0: chair_3, table_8, bench_1
hallway_0: table_6
entryway/foyer/lobby_0: bench_3

Objects in the house:
pillow_0: bed_0
pillow_1: bed_0
apple_0: chair_2
pen_0: table_6
laptop_0: table_1

Task progress:
Agent 0 rearranged the pillow_1 from couch_1 to bed_0.
Agent 1 rearranged the pillow_0 from chair_0 to bed_0.

Your agent's observations of the last executed action (if available):
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Based on the task and the list of objects in the house, the task-relevant objects are pillow_0, pillow_1 and apple_0, located on bed_0, bed_0 and chair_2 respectively. The task requires rearranging pillows first to the desired location of bed in bedroom. After that, apple needs to be rearranged to counter. Based on the object locations provided in the object list and the task progress summary, pillow_0 and pillow_1 have been rearranged to bed_0. Since the apple should be rearranged after pillows, I can now ask my Agent 0 to rearrange apple_0.
Agent_0_Action: Rearrange[apple_0, on, counter_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Example 3:
Task:
Move all towels from the kitchen to the bathroom.

House description:
living_room_0: couch_0, table_0, chair_0, chair_1, chair_2, table_1, chest_of_drawers_0, chest_of_drawers_1
bathroom_0: toilet_0, table_2
kitchen_0: chair_2, cabinet_0, cabinet_1, cabinet_2, cabinet_3, fridge_0, cabinet_4

Objects in the house:
hand_towel_0: table_2
hand_towel_1: bathroom_0
bath_towel_0: table_2
sponge_0: chair_2
pen_0: table_0
stuffed_toy_0: table_1

Task progress:
Agent 0 rearranged the hand_towel_0 from chair to table_2 and bath_towel_0 to table_2.
Agent 1 rearranged the hand_towel_1 to the bathroom_0.

Your agent's observations of the last executed action (if available):
Agent_0_observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Based on the task and the list of objects in the house, the task-relevant objects are hand_towel_0, hand_towel_1 and bath_towel_0, located on table_2, bathroom_0 and table_2 respectively. The task requires moving all towels to the bathroom. Based on the object locations in the list of objects and the task progress, all towels are in the bathroom already and were moved to the bathroom by agent 0 and agent 1. So the task is complete.
Final Thought: Exit!
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Example 4:
Task: Put book on the shelves and apple on the counter.

House description:
living_room_0: couch_0, couch_1, table_1, table_2
bedroom_0: bed_0, table_3, shelves_0
kitchen_1: cabinet_0, table_3, chair_1, chair_2, chair_3, chair_4, counter_0
laundryroom/mudroom_0: washer_dryer_0, washer_dryer_1, shelves_1
bathroom_0: toilet_0

Objects in the house:
book_0: shelves_0
apple_0: counter_0
stuffed_toy_0: bed_0
kettle_0: table_1

Task progress summary:
Agent 0 rearranged book_0 to shelves_0 multiple times.
Agent 1 hasn't taken any actions for the task yet and is currently waiting.

Your agent's observations of the last executed action (if available):
Agent_0_observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Based on the task and the list of objects in the house, the task-relevant objects are book_0 and apple_0, located on shelves_0 and counter_0 respectively. The task requires putting book on the shelves and apple on the counter. Based on the task progress summary, agent 0 has rearranged book on the shelves multiple times. So I should re-verify the location of the task-relevant objects from the list of the objects. Based on the list of objects, book is already on shelves and apple is on the counter. Since this was the requirement of the task, the task is complete.
Final Thought: Exit!
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Task:
{input}

House description:
{house_description}

Objects in the house:
{all_objects}

{summary}

Your agent's observations of the last executed action (if available): {agent0_obs}
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought:

\end{prompt}
\end{mdframed}

==> prompts/multi_agent_react_summary_po.tex <==
\begin{mdframed}[
    linewidth=1pt, % Width of the border line
    linecolor=black, % Color of the border line
    backgroundcolor=gray!10, % Background color of the box
    roundcorner=5pt, % Round cornered box
    frametitle={Multi Agent | ReAct-Summary | Decentralized | Partial Observability},
    frametitlealignment=\center % Center align the frame title
]

\begin{prompt}
<|start_header_id|>system<|end_header_id|>
- Overview:
Your goal is to find the optimal next action for an agent collaborating with another agent in a multi-agent planning task. Find action for the agent as best as you can. The task assigned to you will be situated in a house and will generally involve navigating to objects, picking and placing them on different receptacles to achieve rearrangement. Below is the detailed description of different actions that the agent can use for solving the task. You can assign them to Agent_{id} as required. Remember to assign only 1 action to your agent. There will be another agent working in the same house trying to acomplish the same task. Your role is to enable Agent_{id} to finish the task together by collaborating with its partner agent.

You should account for the task progress, locations of objects in the house, the partner agent's state, and your agent's observations to determine the next optimal action for your agent. The optimal action should be aimed at enabling faster and more efficient task completion. So avoid doing tasks that the partner agent is doing and instead focus on tasks that are left over and can be done in parallel.

{tool_descriptions}
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Here are some examples of allocating optimal next actions to your agent in a given task:

Example 1:
Task:
Move all objects from sofa to bedroom and place them next to the toy truck.

House description:
living_room_0: chair_0, chair_1, chair_2, chair_3, table_0, couch_0, couch_1, table_1, table_2, table_3
closet_0: shelves_0
bedroom_0: bed_0, chest_of_drawers_0, chest_of_drawers_1
kitchen_1: cabinet_0, table_4, chair_4, chair_5, chair_6, chair_7
bedroom_1: bed_1, chest_of_drawers_2, chest_of_drawers_3
bedroom_2: bed_2, chest_of_drawers_4, chest_of_drawers_5, wardrobe_0, wardrobe_1
laundryroom/mudroom_0: washer_dryer_0, washer_dryer_1, shelves_1, shelves_2
bathroom_0: toilet_0
bathroom_2: toilet_1
bathroom_1: toilet_2
kitchen_0: fridge_0
garage_0: fridge_1

Objects found in the house so far:
cherry_0: couch_0
apple_0: couch_0
banana_0: couch_0

Task progress:
Agent 0 is walking.
Agent 1 is waiting and ready to start collaborating.

Your agent's observations of the last executed action (if available):

<|eot_id|>

<|start_header_id|>assistant<|end_header_id|>
Thought: Based on the task and the list of objects in the house, the current task-relevant objects are cherry_0, banana_0, apple_0 located on the couch_0, couch_0, and couch_0 respectively. The desired location for these objects is the bedroom, specifically next to the toy truck based on the task description. So I will choose the bed where toy truck is located as target location for these objects. However, it is unclear which bed is the toy truck on. So I will ask my agent to explore each bedroom with names bedroom_0, bedroom_1, and bedroom_2 in the house one by one. I will assign the "explore" action to the agent using the exact names of the rooms to prevent any confusion for the agent.
Agent_0_Action: Explore[bedroom_0]
Assigned!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 2:
Task:
Move pillow to bed and then move apple to kitchen counter.

House description:
living_room_0: table_0, couch_0, chair_2, shelves_1, chair_5, chair_6, table_7, chair_7, chair_8, chair_9, chair_10, chair_11, chair_12, table_9, table_10, stand_0, chest_of_drawers_2
laundryroom/mudroom_0: washer_dryer_0, washer_dryer_1, shelves_0
bathroom_1: bathtub_0, table_11
bedroom_1: table_1, chair_1, bed_0, table_4, table_5, chair_4, stool_0, bench_0, table_12, chest_of_drawers_3
kitchen_0: cabinet_0, cabinet_1, cabinet_2, counter_0, chair_2, cabinet_3, cabinet_4, cabinet_5, chair_13, chair_14, chair_15, counter_1, cabinet_6, fridge_0, cabinet_7, cabinet_8
bedroom_0: chair_0, table_2, table_3, bed_1, bench_2, chest_of_drawers_0, chest_of_drawers_1
bathroom_0: chair_3, table_8, bench_1
hallway_0: table_6
entryway/foyer/lobby_0: bench_3

Objects found in the house so far:
pillow_0: bed_0
pillow_1: agent_0
laptop_0: table_1

Task progress:
Agent 0 moved the pillow_0 from chair to bed_0 and is currently carrying rearranging pillow_1.
Agent 1 is currently waiting.

Your agent's observations of the last executed action (if available):
Agent_0_observation: Action Rearrange[pillow_1, on, bed_0, None, None] is still in progress.
<|eot_id|>

<|start_header_id|>assistant<|end_header_id|>
Thought: Based on the task and the list of objects in the house, the task-relevant objects are pillow_0 and pillow_1 located on bed_0 and agent_0 respectively and apple, whose location is unknown. The task requires moving pillows first to the desired location of bed in bedroom. Since pillow_0 is already on bed_0, I will focus on pillow_1 and searching for apple. Since Agent 0 is still rearranging the pillow_1 to the bed_0, which needs to be rearranged before rearranging apple, I will let Agent 0 finish this part of the task. So, I will reassign rearange pillow_1 action back to Agent 0.
Agent_0_Action: Rearrange[pillow_1, on, bed_0, None, None]
Assigned!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 3:
Task:
Move all towels from the kitchen to the bathroom.

House description:
living_room_0: couch_0, table_0, chair_0, chair_1, chair_2, table_1, chest_of_drawers_0, chest_of_drawers_1
bathroom_0: toilet_0, table_2
kitchen_0: chair_2, cabinet_0, cabinet_1, cabinet_2, cabinet_3, fridge_0, cabinet_4

Objects found in the house so far:
hand_towel_0: table_2
hand_towel_1: bathroom_0
bath_towel_0: table_2
sponge_0: chair_2
pen_0: table_0
stuffed_toy_0: table_1

Task progress:
Agent 0 moved the hand_towel_0 from chair to table_2. Agent 0 moved bath_towel_0 to table_2.
Agent 1 moved the hand_towel_1 to the bathroom_0.

Your agent's observations of the last executed action (if available):
Agent_0_observation: Successfull execution!
<|eot_id|>

<|start_header_id|>assistant<|end_header_id|>
Thought: Based on the task and the list of objects in the house, the task-relevant objects are hand_towel_0, hand_towel_1 and bath_towel_0, located on table_2, bathroom_0 and table_2 respectively. All agents have finished successful execution. Since the task is to move all towels to the bathroom and all towels are in the bathroom already and no towels are in the kitchen, the task is complete.
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 4:
Task:
Place stuffed toy and book on the shelves.

House description:
living_room_0: table_0, couch_0, chair_2, shelves_1, chair_5, chair_6, table_7, chair_7, chair_8, chair_9, chair_10, chair_11, chair_12, table_9, table_10, stand_0, chest_of_drawers_2
laundryroom/mudroom_0: washer_dryer_0, washer_dryer_1, shelves_0
bedroom_0: chair_0, table_2, table_3, bed_1, bench_2, chest_of_drawers_0, chest_of_drawers_1
bathroom_0: toilet_0
bathroom_2: toilet_1
kitchen_0: fridge_0

Objects found in the house so far:

Task progress:
Agent 0 is currently waiting and ready to start collaborating.
Agent 1 is currently waiting and ready to start collaborating.

Your agent's observations of the last executed action (if available):
Agent_0_Observation: Node with name living room not present in the graph. The entity name may be wrong or the entity may not exist in the house. Use entity names that match with the names of rooms and furniture provided in the house description.
<|eot_id|>

<|start_header_id|>assistant<|end_header_id|>
Thought: Based on the task and the list of objects in the house, the task-relevant objects are stuffed toy and book. The task requires moving them to the desired location of shelves either in the living room or the laundryroom. Since it is unclear where stuffed toy and book are in the house, I will first ask my agent 0 to search the rooms in the house that are likely to have stuffed toy and book. From the house description, living room and bedroom are likely to have these objects. So, I will ask my agent 0 to explore the living room. Based on my agent's previous observation, it looks like the living room name used with the agent's previous action did not match the house description. So I will use the EXACT name of the living room provided in the house description when I assign action to my agent.
Agent_0_Action: Explore[living_room_0]
Assigned!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 5:
Task:
Put laptop and pen next to each other on the bed.

House description:
living_room_0: chair_0, chair_1, chair_2, chair_3, table_0, couch_0, couch_1, table_1, table_2, table_3
bathroom_1: bathtub_0, table_11
bedroom_1: chair_1, bed_0, table_4, table_5, chair_4, stool_0, bench_0, table_12, chest_of_drawers_3
kitchen_0: cabinet_0, cabinet_1, cabinet_2, counter_0, chair_2, cabinet_3, cabinet_4, cabinet_5, chair_13, chair_14, chair_15, counter_1, cabinet_6, fridge_0, cabinet_7, cabinet_8
bedroom_0: chair_0, table_2, table_3, bed_1, bench_2, chest_of_drawers_0, chest_of_drawers_1
bathroom_0: chair_3, table_8, bench_1
hallway_0: table_6

Objects found in the house so far:
apple_0: chair_2
pen_0: table_6
laptop_0: table_1

Task progress:
Agent 0 walked around and is currently waiting.
Agent 1 is currently walking.

Your agent's observations of the last executed action (if available):
<|eot_id|>

<|start_header_id|>assistant<|end_header_id|>
Thought: Based on the task and the list of objects in the house, the task-relevant objects are laptop_0 and pen_0, located on table_1 and table_6 respectively. The task requires moving them to the desired location of bed in bedroom. Since the laptop and pen need to be placed next to each other and Agent 1 hasn't started the task yet, I will wait for the agent 1 to place one of them on the bed first and ask my agent 0 to wait.
Agent_0_Action: Wait[]
Assigned!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 6:
Task:
Let's clear the plate and glasses from the living room table. Move them to the counter and place them next to each other.

House description:
living_room_0: couch_0, table_0, chair_0, chair_1, chair_2, table_1, chest_of_drawers_0, chest_of_drawers_1
bathroom_0: toilet_0, table_2
kitchen_0: cabinet_0, cabinet_1, cabinet_2, counter_0, chair_2, cabinet_3, cabinet_4, cabinet_5, chair_13, chair_14, chair_15, counter_1, cabinet_6, fridge_0, cabinet_7, cabinet_8
bedroom_0: chair_0, table_2, table_3, bed_1, bench_2, chest_of_drawers_0, chest_of_drawers_1

Objects found in the house so far:
plate_0: table_1
drinkware_0: counter_0
drinkware_1: table_1
lamp_0: table_1

Task progress:
Agent 0 moved drinkware_0 to the counter and is currently walking.
Agent 1 is currently walking.

Your agent's observations of the last executed action (if available):
<|eot_id|>

<|start_header_id|>assistant<|end_header_id|>
Thought: Based on the task and the list of objects in the house, the task-relevant objects are plate_0, drinkware_0, and drinkware_1 located on table_1, counter_0, and table_1 respectively. The task requires moving them to the desired location of counter next to each other. Since the one of the drinkware was already moved to the counter, I will ask my agent 0 to move the remaining plate next to the glass on the counter.
Agent_0_Action: Rearrange[plate_0, on, counter_0, next_to, drinkware_0]
Assigned!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Task:
{input}

House description:
{house_description}

Objects found in the house so far:
{all_objects}

{summary}

Your agent's observations of the last executed action (if available): {agent0_obs}
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought:
\end{prompt}
\end{mdframed}

==> prompts/multi_agent_react_tools_fo.tex <==
\begin{mdframed}[
    linewidth=1pt, % Width of the border line
    linecolor=black, % Color of the border line
    backgroundcolor=gray!10, % Background color of the box
    roundcorner=5pt, % Round cornered box
    frametitle={Multi Agent | ReAct-Tools | Decentralized | Full Observability \\ ( Used to simulate synthetic human in full observability settings )},
    frametitlealignment=\center % Center align the frame title
]

\begin{prompt}

<|start_header_id|>system<|end_header_id|>
- Overview:
Solve the given planning problem as best as you can. The task assigned to you will be situated in a house and will generally involve navigating to objects, picking and placing them on different receptacles to achieve rearrangement. Below is the detailed description of the actions you can use for solving the task. You can assign them to Agent_{id} as required. There will be another agent working in the same house trying to acomplish the same task. Your role is to finish the task together by collaborating.

{agent_descriptions}
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Here are some examples:

Example 1:
Task: Move all objects from sofa to sink
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find the objects that are on the sofa.
Agent_{id}_Action: FindObjectTool[Objects on the sofa]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - cherry_0 in Sofa
- banana_0 in Sofa
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found task relevant objects, I will ask it to find task relevant target receptacles.
Agent_{id}_Action: FindReceptacleTool[sink]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: sink_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both task relevant objects and receptacles have been found, I will enquire the actions of the other agent.
Agent_{id}_Action: FindAgentActionTool[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: The agent walked to cherry_0, picked it and placed it on sink_0, and now is standing.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the other agent already moved the cherry_0, I will do the remaining parts of the task.
Agent_{id}_Action: Rearrange[banana_0, on, sink_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Assuming that the other agent finished its actions, all objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 2:
Task: Move pillow to bed and then move apple to kitchen counter
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find the pillow.
Agent_{id}_Action: FindObjectTool[pillow]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - pillow_0 in sofa
- pillow_1 in couch
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found task relevant objects, I will ask it to find task relevant target receptacles.
Agent_{id}_Action: FindReceptacleTool[bed]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: bed_0, bed_1
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both task relevant objects and receptacles have been found, I will enquire the actions of the other agent.
Agent_{id}_Action: FindAgentActionTool[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: The agent is holding pillow_0 and moving.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the other agent seems to be helping with moving pillow_0, I will do the remaining parts of the task. Since there are multiple beds, I will pick any one of them.
Agent_{id}_Action: Rearrange[pillow_1, on, bed_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the target. I will check the actions of the other agent.
Agent_{id}_Action: FindAgentActionTool[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Agent moved pillow_0 to bed_0 and now is walking with apple_0.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Other agent has already moved the pillow and now seems to be moving apple_0. Assuming that the other agent finishes its actions, all objects would be successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 3:
Task: Move bowl, cup and basket to the chair in living room
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find the bowl, cup and basket
Agent_{id}_Action: FindObjectTool[bowl, cup, basket]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - bowl_0 on Sofa
- cup_1 on Sofa
- basket_2 on Sofa
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found task relevant objects, I will ask it to find task relevant target receptacles.
Agent_{id}_Action: FindReceptacleTool[chair in living room]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: chair_0, chair_1, chair_2, chair_3 found in living room.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both task relevant objects and receptacles have been found, I will find the actions of the other agent.
Agent_{id}_Action: FindAgentActionTool[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Agent is walking.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the other agent is walking, I will assume that it is trying to move bowl_0. I will do the next part of the task. Since there are many chairs, I will pick any one of them.
Agent_{id}_Action: Rearrange[cup_1, on, chair_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the target. So I will check again the actions of the other agent.
Agent_{id}_Action: FindAgentActionTool[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Agent is holding bowl_0 and walking.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the other agent is still seems to be moving bowl_0, I will proceed to the next parts of the task.
Agent_{id}_Action: Rearrange[basket_2, on, chair_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Assuming that the other agent finished its actions, all objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 4:
Task: Go on the kitchen table and pick up plate and place it next to drinkware on chair
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find plate on the kitchen table.
Agent_{id}_Action: FindObjectTool[plate on kitchen table]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - plate_0 on kitchen_table_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found the plate on the kitchen table, I will find the actions of the other agent.
Agent_{id}_Action: FindAgentActionTool[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Agent is standing.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the other agent is standing, I will take care of moving the plate to the chair. First I will find the chair.
Agent_{id}_Action: FindReceptacleTool[chair]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: chair_0 found in kitchen.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the chair is found, I will find drinkware on the chair.
Agent_{id}_Action: FindObjectTool[drinkware on the chair]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - drinkware_0 on chair_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the drinkware is found, I will move the plate to the chair next to drinkware.
Agent_{id}_Action: Rearrange[plate_0, on, chair_0, next_to, drinkware_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the the object. Assuming the other agent finished its action, all objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Task: {input}
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought:
\end{prompt}
\end{mdframed}

==> prompts/multi_agent_react_tools_fo_centralized.tex <==
\begin{mdframed}[
    linewidth=1pt, % Width of the border line
    linecolor=black, % Color of the border line
    backgroundcolor=gray!10, % Background color of the box
    roundcorner=5pt, % Round cornered box
    frametitle={Multi Agent | ReAct-Tools | Centralized | Full Observability},
    frametitlealignment=\center % Center align the frame title
]

\begin{prompt}
<|start_header_id|>system<|end_header_id|>
- Overview:
Solve the given multi-agent planning problem as best as you can. The task assigned to you will be situated in a house and will generally involve navigating to objects, picking and placing them on different receptacles to achieve rearrangement. Below is the detailed description of the actions you can use for solving the task. You can assign them to Agent_0 and/or Agent_1 as required.

{tool_descriptions}
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Here are some examples:

Example 1:
Task: Move all objects from sofa to sink
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask one agent to find the objects that are on the sofa. In parallel, I should ask the other to find the sink.
Agent_0_Action: FindObjectTool[Objects on the sofa]
Agent_1_Action: FindReceptacleTool[sink]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_Observation: - cherry_0 in Sofa
- banana_0 in Sofa
Agent_1_Observation: sink_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both agents have found the task relevant objects and receptacles, I will come up with a task plan.
Agent_0_Action: Rearrange[cherry_0, on, sink_0, None, None]
Agent_1_Action: Rearrange[banana_0, on, sink_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_Observation: Successful execution!
Agent_1_Observation: Action "Rearrange[banana_0, on, sink_0, None, None]" is still in progress.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent 0 successfully transferred the target. Agent 1 is still executing the previous action, so I will reassign the same action to it.
Agent_0_Action: Wait[]
Agent_1_Action: Rearrange[banana_0, on, sink_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_Observation: Waiting
Agent_1_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: All objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 2:
Task: Move pillow to bed and then move apple to kitchen counter
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask one agent to find the pillow. In parallel, I should ask the other to find bed.
Agent_0_Action: FindObjectTool[pillow]
Agent_1_Action: FindReceptacleTool[bed]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_Observation: - pillow_0 in sofa
- pillow_1 in couch
Agent_1_Observation: bed_0, bed_1
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both agents have found the task relevant objects and receptacles, I will come up with a task plan. Since there are many beds, I will pick any one of them.
Agent_0_Action: Rearrange[pillow_0, on, bed_0, None, None]
Agent_1_Action: Rearrange[pillow_1, on, bed_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_Observation: Successful execution!
Agent_1_Observation: Action "Rearrange[pillow_1, on, bed_0, None, None]" is still in progress.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent 0 successfully transferred the target. Agent 1 is still executing the previous action, so I will reassign the same action to it.
Agent_0_Action: Wait[]
Agent_1_Action: Rearrange[pillow_1, on, bed_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_Observation: Waiting
Agent_1_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both pillows have been successfully moved, I will move on to the next part of the task. I should ask one agent to find the apple. In parallel, I should ask the other to find kitchen counter.
Agent_0_Action: FindObjectTool[apple]
Agent_1_Action: FindReceptacleTool[kitchen counter]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_Observation: - apple_0 in sofa
Agent_1_Observation: counter_0, counter_1, counter_2 are in kitchen
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both agents have found the task relevant objects and receptacles, I will come up with a task plan. Since there are multiple counters in kitchen, I will pick any one of them.
Agent_0_Action: Rearrange[apple_0, on, counter_0, None, None]
Agent_1_Action: Wait[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_Observation: Successful execution!
Agent_1_Observation: Waiting
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: All objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 3:
Task: Move bowl, cup and basket to the chair in living room
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask one agent to find bowl, cup and basket. In parallel, I should ask the other to find the chair in living room.
Agent_0_Action: FindObjectTool[bowl, cup, basket]
Agent_1_Action: FindReceptacleTool[chair in living room]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_Observation: - bowl_0 in Sofa
- cup_1 in Sofa
- basket_2 in Sofa
Agent_1_Observation: chair_0, chair_1, chair_2, chair_3 found in living room.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both agents have found the task relevant objects and receptacles, I will come up with a task plan. Since there are many chairs, I will pick any one of them.
Agent_0_Action: Rearrange[bowl_0, on, chair_0, None, None]
Agent_1_Action: Rearrange[cup_1, on, chair_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_Observation: Successful execution!
Agent_1_Observation: Action "Rearrange[banana_0, on, sink_0, None, None]" is still in progress.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent 0 successfully transferred the target. So I will assign next action to it. Agent 1 is still executing the previous action, so I will reassign the same action to it.
Agent_0_Action: Rearrange[basket_2, on, chair_0, None, None]
Agent_1_Action: Rearrange[cup_1, on, chair_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_Observation: Action "Rearrange[basket_2, on, chair_0, None, None]" is still in progress.
Agent_1_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent 1 successfully transferred the target. Agent 0 is still executing the previous action, so I will reassign the same action to it.
Agent_0_Action: Rearrange[basket_2, on, chair_0, None, None]
Agent_1_Action: Wait[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_Observation: Successful execution!
Agent_1_Observation: Waiting
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: All objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 4:
Task: Go on the kitchen table and pick up plate and place it next to drinkware on chair
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask one agent to find plate on the kitchen table, and other agent to find the drinkware on chair.
Agent_0_Action: FindObjectTool[plate on kitchen table]
Agent_1_Action: FindObjectTool[drinkware on chair]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_observation: - plate_0 on kitchen_table_0
Agent_1_observation: - drinkware_0 on chair_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both the task relevant objects and receptacles have been found I will ask one agent to move the palte next to the drinkware.
Agent_0_Action: Rearrange[plate_0, on, chair_0, next_to, drinkware_0]
Agent_1_Action: Wait[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_0_Observation: Successful execution!
Agent_1_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: All objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Task: {input}
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought:
\end{prompt}
\end{mdframed}

==> prompts/multi_agent_react_tools_po.tex <==
\begin{mdframed}[
    linewidth=1pt, % Width of the border line
    linecolor=black, % Color of the border line
    backgroundcolor=gray!10, % Background color of the box
    roundcorner=5pt, % Round cornered box
    frametitle={Multi Agent | ReAct-Tools | Decentralized | Partial Observability \\ ( Used to simulate synthetic human in partial observability settings )},
    frametitlealignment=\center % Center align the frame title
]

\begin{prompt}

<|start_header_id|>system<|end_header_id|>
- Overview:
Solve the given planning problem as best as you can. The task assigned to you will be situated in a house and will generally involve navigating to objects, picking and placing them on different receptacles to achieve rearrangement. Below is the detailed description of the actions you can use for solving the task. You can assign them to Agent_{id} as required. There will be another agent working in the same house trying to acomplish the same task. your role is to finish the task together by collaborating.

{agent_descriptions}
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Here are some examples:

Example 1:
Task: Move all objects from the kitchen table to sink
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find objects on the kitchen table
Agent_{id}_Action: FindObjectTool[objects on kitchen table]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: No such object yet found.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since these objects are not found, I should search for them. I will ask the agent to find the kitchen table.
Agent_{id}_Action: FindReceptacleTool[kitchen table]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: kitchen_table_0 found in kitchen.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the kitchen table is found, I will navigate to it.
Agent_{id}_Action: Navigate[kitchen_table_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that I am near the kitchen table, I will again try to find objects on it.
Agent_{id}_Action: FindObjectTool[objects on kitchen table]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - spoon_0 on kitchen_table_0
- pan_1 on kitchen_table_0
- spatula_2 on kitchen_table_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found objects on the kitchen table, I will find the actions of the other agent.
Agent_{id}_Action: FindAgentActionTool[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Agent is walking with while holding spoon_0.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the other agent is walking with spoon_0, I will assume it will take care of moving the pan to the sink. I will move to the next object.
Agent_{id}_Action: FindReceptacleTool[sink]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: sink_0 found in kitchen.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the sink is found, I will move the pan to the sink.
Agent_{id}_Action: Rearrange[pan_1, on, sink_0, none, none]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the pan. I will check what the other agent is doing before moving the spatula.
Agent_{id}_Action: FindAgentActionTool[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Agent put spoon_0 in sink and now is standing.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the other agent has finished its action, I will move the spatula to the sink.
Agent_{id}_Action: Rearrange[spatula_2, on, sink_0, none, none]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the the object. Assuming the other agent finished its action, all objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 2:
Task: Move ball, cup and phone to the chair in living room
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find the ball, cup and phone
Agent_{id}_Action: FindObjectTool[ball, cup, phone]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: No such object yet found.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since these objects are not found, I should search for them. I will ask the agent to find relevant rooms for these objects.
Agent_{id}_Action: FindRoomTool[room that may have ball, cup, and phone]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: kitchen_0, living_room_0.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now I know which rooms may have these objects, I should ask the agent to explore them.
Agent_{id}_Action: Explore[kitchen_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the the agent successufully explored the room, I will again try to find the objects.
Agent_{id}_Action: FindObjectTool[ball, cup, phone]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - ball_0 on kitchen counter
- cup_1 on kitchen counter
- phone_2 on kitchen counter
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found task relevant objects, I will ask it to find task relevant target receptacles.
Agent_{id}_Action: FindReceptacleTool[chair in living room]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: chair_0, chair_1, chair_2, chair_3 found in living room.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both task relevant objects and receptacles have been found, I will find the actions of the other agent.
Agent_{id}_Action: FindAgentActionTool[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Agent is walking with ball_0.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the other agent is walking with ball_0, I will do the next part of the task. Since there are many chairs, I will pick any one of them.
Agent_{id}_Action: Rearrange[cup_1, on, chair_0, none, none]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the target. So I will check again the actions of the other agent.
Agent_{id}_Action: FindAgentActionTool[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Agent is holding ball_0 and walking.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the other agent is still seems to be moving ball_0, I will proceed to the next parts of the task.
Agent_{id}_Action: Rearrange[phone_2, on, chair_0, none, none]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Assuming that the other agent finished its actions, all objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 3:
Task: Move pillow to bed and then move apple to kitchen counter.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find the pillow and apple.
Agent_{id}_Action: FindObjectTool[pillow, apple]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: No such object yet found.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since these objects are not found, I should search for them. I will ask the agent to find relevant rooms for these objects.
Agent_{id}_Action: FindRoomTool[room that may have pillow and apple]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: bedroom_0, living_room_0, kitchen_0.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now I know which rooms may have these objects, I should ask the agent to explore them.
Agent_{id}_Action: Explore[living_room_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the agent successfully explored the room, I will again try to find the objects.
Agent_{id}_Action: FindObjectTool[pillow, apple]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - pillow_0 on couch_0
- apple_1 on coffee table_2
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found task relevant objects, I will ask it to find task relevant target receptacles.
Agent_{id}_Action: FindReceptacleTool[bed in bedroom]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: bed_0 found in bedroom.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both task relevant objects and receptacles have been found, I will find the actions of the other agent.
Agent_{id}_Action: FindAgentActionTool[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Agent is walking with while holding pillow_0.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the other agent is walking with pillow_0, I will assume it will take care of moving the pillow to the bed. I will move to the next part of the task.
Agent_{id}_Action: FindReceptacleTool[kitchen counter]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: kitchen_counter_0 found in kitchen.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the kitchen counter is found, I will move the apple to the kitchen counter.
Agent_{id}_Action: Rearrange[apple_1, on, kitchen_counter_0, none, none]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the apple. Assuming the other agent finished its action, all objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 4:
Task: Go on the kitchen table and pick up plate and place it next to drinkware on chair
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find the plate on the kitchen table.
Agent_{id}_Action: FindObjectTool[plate on kitchen table]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: No such object yet found.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since these objects are not found, I should search for them. I will ask the agent to find the kitchen table.
Agent_{id}_Action: FindReceptacleTool[kitchen table]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: kitchen_table_0 found in kitchen.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the kitchen table is found, I will navigate to it.
Agent_{id}_Action: Navigate[kitchen_table_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that I am near the kitchen table, I will again try to find objects on it.
Agent_{id}_Action: FindObjectTool[plate on kitchen table]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - plate_0 on kitchen_table_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found the plate on the kitchen table, I will find the actions of the other agent.
Agent_{id}_Action: FindAgentActionTool[]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Agent is standing.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the other agent is standing, I will take care of moving the plate to the chair. First I will find the chair.
Agent_{id}_Action: FindReceptacleTool[chair]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: chair_0 found in kitchen.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the chair is found, I will find drinkware on the chair.
Agent_{id}_Action: FindObjectTool[drinkware on the chair]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - drinkware_0 on chair_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the drinkware is found, I will move the plate to the chair next to drinkware.
Agent_{id}_Action: Rearrange[plate_0, on, chair_0, next_to, drinkware_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the the object. Assuming the other agent finished its action, all objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Task: {input}
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought:
\end{prompt}
\end{mdframed}

==> prompts/single_agent_react_tools_fo.tex <==
\begin{mdframed}[
    linewidth=1pt, % Width of the border line
    linecolor=black, % Color of the border line
    backgroundcolor=gray!10, % Background color of the box
    roundcorner=5pt, % Round cornered box
    frametitle={Single Agent | ReAct-Tools | Full Observability },
    frametitlealignment=\center % Center align the frame title
]

\begin{prompt}
<|start_header_id|>system<|end_header_id|>
- Overview:
Solve the given planning problem as best as you can. The task assigned to you will be situated in a house and will generally involve navigating to objects, picking and placing them on different receptacles to achieve rearrangement. Below is the detailed description of the actions you can use for solving the task. You can assign them to Agent_{id} as required.

{tool_descriptions}
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Here are some examples:

Example 1:
Task: Move all objects from the kitchen table to sink
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find objects on the kitchen table
Agent_{id}_Action: FindObjectTool[objects on kitchen table]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - plate_0 on kitchen_table_0
- bowl_1 on kitchen_table_0
- cup_2 on kitchen_table_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found task relevant objects, I will ask it to find task relevant target receptacles.
Agent_{id}_Action: FindReceptacleTool[sink]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: sink_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both task relevant objects and receptacles have been found, I will assign action to the agent.
Agent_{id}_Action: Rearrange[plate_0, on, sink_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the target. I will assign next action to the agent.
Agent_{id}_Action: Rearrange[bowl_1, on, sink_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the target. I will assign next action to the agent.
Agent_{id}_Action: Rearrange[cup_2, on, sink_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: All objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 2:
Task: Move pillow to bed and then move apple to kitchen counter
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should the agent to find the pillow.
Agent_{id}_Action: FindObjectTool[pillow]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - pillow_0 in sofa
- pillow_1 in couch
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found task relevant objects, I will ask it to find task relevant target receptacles.
Agent_{id}_Action: FindReceptacleTool[bed]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: bed_0, bed_1
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both task relevant objects and receptacles have been found, I will assign action to the agent. Since there are many beds, I will pick any one of them.
Agent_{id}_Action: Rearrange[pillow_0, on, bed_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the target. I will assign next action to the agent.
Agent_{id}_Action: Rearrange[pillow_1, on, bed_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both pillows have been successfully moved, I will move on to the next part of the task. I should ask the agent to find the apple.
Agent_{id}_Action: FindObjectTool[apple]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - apple_0 in sofa
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found task relevant objects, I will ask it to find task relevant target receptacles.
Agent_{id}_Action: FindReceptacleTool[kitchen counter]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: counter_0, counter_1, counter_2 are in kitchen
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both task relevant objects and receptacles have been found, I will assign action to the agent. Since there are multiple counters in kitchen, I will pick any one of them.
Agent_{id}_Action: Rearrange[apple_0, on, counter_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: All objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 3:
Task: Move bowl, cup and basket to the chair in living room
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask one agent to find the bowl, cup and basket
Agent_{id}_Action: FindObjectTool[bowl, cup, basket]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - bowl_0 on Sofa
- cup_1 on Sofa
- basket_2 on Sofa
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found task relevant objects, I will ask it to find task relevant target receptacles.
Agent_{id}_Action: FindReceptacleTool[chair in living room]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: chair_0, chair_1, chair_2, chair_3 found in living room.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both task relevant objects and receptacles have been found, I will assign action to the agent. Since there are many chairs, I will pick any one of them.
Agent_{id}_Action: Rearrange[bowl_0, on, chair_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the target. So I will assign next action to it.
Agent_{id}_Action: Rearrange[cup_1, on, chair_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the target. So I will assign next action to it.
Agent_{id}_Action: Rearrange[basket_2, on, chair_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: All objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 4:
Task: Go on the kitchen table and pick up plate and place it next to drinkware on chair
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find plate on the kitchen table and drinkware on the chair
Agent_{id}_Action: FindObjectTool[plate on kitchen table and drinkware on chair]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - plate_0 on kitchen_table_0
- drinkware_0 on chair_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that I found objects on the kitchen table and chair, I will ask the agent to navigate to the kitchen table.
Agent_{id}_Action: Navigate[kitchen_table_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that I am near the kitchen table, I will take care of moving the plate to the chair and place it next to drinkware.
Agent_{id}_Action: Rearrange[plate_0, on, chair_0, next_to, drinkware_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the the object. All objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Task: {input}
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought:

\end{prompt}
\end{mdframed}

==> prompts/single_agent_react_tools_po.tex <==
\begin{mdframed}[
    linewidth=1pt, % Width of the border line
    linecolor=black, % Color of the border line
    backgroundcolor=gray!10, % Background color of the box
    roundcorner=5pt, % Round cornered box
    frametitle={Single Agent | ReAct-Tools | Partial Observability},
    frametitlealignment=\center % Center align the frame title
]

\begin{prompt}
<|start_header_id|>system<|end_header_id|>
- Overview:
Solve the given planning problem as best as you can. The task assigned to you will be situated in a house and will generally involve navigating to objects, picking and placing them on different receptacles to achieve rearrangement. Below is the detailed description of the actions you can use for solving the task. You can assign them to Agent_{id} as required.

{tool_descriptions}
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Here are some examples:
Example 1:
Task: Move all objects from the kitchen table to sink
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find objects on the kitchen table
Agent_{id}_Action: FindObjectTool[objects on kitchen table]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: No such object yet found.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since these objects are not found, I should search for them. I will ask the agent to find the kitchen table.
Agent_{id}_Action: FindReceptacleTool[kitchen table]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: kitchen_table_0 found in kitchen.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the kitchen table is found, I will navigate to it.
Agent_{id}_Action: Navigate[kitchen_table_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that I am near the kitchen table, I will again try to find objects on it.
Agent_{id}_Action: FindObjectTool[objects on kitchen table]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - plate_0 on kitchen_table_0
- bowl_1 on kitchen_table_0
- cup_2 on kitchen_table_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found objects on the kitchen table, I will ask it to find sink.
Agent_{id}_Action: FindReceptacleTool[sink]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: sink_0 found in kitchen.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the sink is found, I will ask the agent to start moving objects to it.
Agent_{id}_Action: Rearrange[plate_0, on, sink_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the target. I will assign next action to the agent.
Agent_{id}_Action: Rearrange[bowl_1, on, sink_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the target. I will assign next action to the agent.
Agent_{id}_Action: Rearrange[cup_2, on, sink_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: All objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 2:
Task: Move pillow to bed and then move apple to kitchen counter.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find the pillow and apple.
Agent_{id}_Action: FindObjectTool[pillow, apple]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: No such object yet found.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since these objects are not found, I should search for them. I will ask the agent to find relevant rooms for these objects.
Agent_{id}_Action: FindRoomTool[room that may have pillow and apple]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: bedroom_0, living_room_0, kitchen_0.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now I know which rooms may have these objects, I should ask the agent to explore them.
Agent_{id}_Action: Explore[living_room_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the agent successfully explored the room, I will again try to find the objects.
Agent_{id}_Action: FindObjectTool[pillow, apple]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - pillow_0 on couch_0
- apple_1 on coffee table_2
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found task relevant objects, I will ask it to find task relevant target receptacles.
Agent_{id}_Action: FindReceptacleTool[bed in bedroom]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: bed_0 found in bedroom.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both task relevant objects and receptacles have been found, I will assign action to the agent. Since there are many beds, I will pick any one of them.
Agent_{id}_Action: Rearrange[pillow_0, on, bed_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the target. I will assign next action to the agent.
Agent_{id}_Action: Rearrange[pillow_1, on, bed_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both pillows have been successfully moved, I will move on to the next part of the task. I will ask agent to find kitchen counter.
Agent_{id}_Action: FindReceptacleTool[kitchen counter]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: counter_0, counter_1, counter_2 are in kitchen
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: I will assign action to the agent. Since there are multiple counters in kitchen, I will pick any one of them.
Agent_{id}_Action: Rearrange[apple_0, on, counter_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: All objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>


<|start_header_id|>user<|end_header_id|>
Example 3:
Task: Move bowl, cup and basket to the chair in living room
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find the bowl, cup and basket
Agent_{id}_Action: FindObjectTool[bowl, cup, basket]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: No such object yet found.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since these objects are not found, I should search for them. I will ask the agent to find relevant rooms for these objects.
Agent_{id}_Action: FindRoomTool[room that may have bowl, cup, and basket]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: kitchen_0, living_room_0.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now I know which rooms may have these objects, I should ask the agent to explore them.
Agent_{id}_Action: Explore[kitchen_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since the the agent successufully explored the room, I will again try to find the objects.
Agent_{id}_Action: FindObjectTool[bowl, cup, basket]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - bowl_0 on kitchen counter
- cup_1 on kitchen counter
- basket_2 on kitchen counter
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found task relevant objects, I will ask it to find task relevant target receptacles.
Agent_{id}_Action: FindReceptacleTool[chair in living room]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: chair_0, chair_1, chair_2, chair_3 found in living room.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both task relevant objects and receptacles have been found, I will assign action to the agent. Since there are many chairs, I will pick any one of them.
Agent_{id}_Action: Rearrange[bowl_0, on, chair_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the target. So I will assign next action to it.
Agent_{id}_Action: Rearrange[cup_1, on, chair_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the target. So I will assign next action to it.
Agent_{id}_Action: Rearrange[basket_2, on, chair_0, None, None]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: All objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Example 4:
Task: Go on the kitchen table and pick up plate and place it next to drinkware on chair
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: First I should ask the agent to find plate on the kitchen table
Agent_{id}_Action: FindObjectTool[plate on kitchen table and drinkware on chair]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: No such objects yet found.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Since these objects are not found, I should search for them. I will ask the agent to find the kitchen table.
Agent_{id}_Action: FindReceptacleTool[kitchen table]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: kitchen_table_0 found in kitchen.
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the kitchen table is found, I will navigate to it.
Agent_{id}_Action: Navigate[kitchen_table_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that I am near the kitchen table, I will again try to find the plate on it.
Agent_{id}_Action: FindObjectTool[plate on kitchen table]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - plate_0 on kitchen_table_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that the agent has found the plate on the kitchen table, I will ask it to find drinkware on the chair.
Agent_{id}_Action: FindObjectTool[drinkware on chair]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_observation: - drinkware_0 on chair_0
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Now that both plate and drinkware have been found, I will take care of moving the plate to the chair next to the drinkware.
Agent_{id}_Action: Rearrange[plate_0, on, chair_0, next_to, drinkware_0]
Assigned!
<|eot_id|>
<|start_header_id|>user<|end_header_id|>
Agent_{id}_Observation: Successful execution!
<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
Thought: Agent successfully transferred the the object. All objects were successfully moved, so I am done!
Final Thought: Exit!
<|eot_id|>

<|start_header_id|>user<|end_header_id|>
Task: {input}
<|start_header_id|>assistant<|end_header_id|>
Thought:

\end{prompt}
\end{mdframed}

==> tables/hallucination-analysis.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[htbp]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
\textbf{Method} & \textbf{Agent} & \textbf{Controllability} & \textbf{Skills} & \textbf{Observability} & \textbf{\begin{tabular}[c]{@{}c@{}}Object\\ Hallucinations \%\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Action \\ Hallucinations \%\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Syntax\\ Errors \%\end{tabular}} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
ReAct-Tools & Single & - & Oracle & Full & 2.52 & 0.01 & 0.33 \\
ReAct-Tools & Multi & Centralized & Oracle & Full & 1.74 & 0.00 & 0.41 \\
ReAct-Tools & Multi & Decentralized & Oracle & Full & 1.08 & 0.00 & 0.08 \\
ReAct-Summary & Multi & Decentralized & Oracle & Full & 1.64 & 0.00 & 14.67 \\ \midrule
\rowcolor[HTML]{EFEFEF} 
ReAct-Tools & Single & - & Oracle & Partial & 5.82 & 0.17 & 0.73 \\
ReAct-Tools & Multi & Decentralized & Oracle & Partial & 6.68 & 0.15 & 1.81 \\
ReAct-Tools & Multi & Decentralized & Learned & Partial & 5.61 & 0.11 & 2.02 \\
ReAct-Tools + RAG & Multi & Decentralized & Oracle & Partial & 4.76 & 0.16 & 0.95 \\
ReAct-Summary & Multi & Decentralized & Oracle & Partial & 4.56 & 1.01 & 43.08 \\
Finetuned-Summary & Multi & Decentralized & Oracle & Partial & 5.29 & 1.01 & 0.00 \\ \bottomrule
\end{tabular}%
}
\vspace{3pt}
\caption{\textbf{Hallucination.} We categorize object hallucination, action hallucination, and syntax errors in our planners. Each error cell indicates percent of actions generated by a planner with corresponding hallucinations averaged across all episodes for the robot agent.}
\label{tab:hallucination}
\end{table}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % This table counts errors for ONLY robot
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[h]
% \begin{adjustbox}{width=\linewidth,center}
% \centering
% % \begin{table}[t]
% % \centering
% \small
% \begin{tabular}{@{}cccccccc@{}}
% \toprule
%          \textbf{Method}& \textbf{Agent}& \makecell{\textbf{Perception} \\ \textbf{Tools}} & \textbf{Skills}& \textbf{Obs.}&  \makecell{\textbf{Object} \\ \textbf{Hallucinations} \(\%\)}& \makecell{\textbf{Action} \\ \textbf{Hallucinations} \(\%\)}& \makecell{\textbf{Syntax} \\ \textbf{Errors} \(\%\)} \\
% \midrule
%          Centralized & Single& Yes & Oracle & Full & 2.52 & 0.01 & 0.33 \\
%          Centralized & Single& Yes &Oracle & Partial & 5.82 & 0.17 & 0.73 \\
%          Centralized & Multi& Yes &Oracle  & Full  & 1.74 & 0.00 & 0.41 \\
%          Decentralized & Multi& Yes &Oracle & Full & 1.08 & 0.00 & 0.08 \\
%          Decentralized & Multi& Yes &Oracle & Partial & 6.68 & 0.15 & 1.81 \\
%          Decentralized & Multi& Yes &Learned & Partial & 5.61 & 0.11 & 2.02 \\
%          Decentralized+RAG & Multi& Yes &Oracle & Partial & 4.76 & 0.16 & 0.95 \\
%          Decentralized & Multi& No &Oracle & Full & 1.64 & 0.00 & 14.67 \\
%          Decentralized & Multi& No &Oracle & Partial & 4.56 & 1.01 & 43.08 \\      
%          Decentralized (FT) & Multi& No& Oracle & Partial & 5.29 & 1.01 & 0.00 \\
% \bottomrule
% \end{tabular}
% % \end{table}
% \end{adjustbox}
% \vspace{3pt} 
% \caption{Hallucination counts for different planner configurations, categorized by object hallucination, action hallucination, and syntax errors. Each error cell indicates percent of assigned actions with respective hallucinations averaged across all episodes for the robot agent.}
% \label{tab:hallucination}
% \end{table}

==> tables/physical-errors.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% % \usepackage[table,xcdraw]{xcolor}
% % Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[h]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}ccccccccc@{}}
% \toprule
% \textbf{Method} & \textbf{Agent} & \textbf{Controllability} & \textbf{Skills} & \textbf{Observability} & \textbf{\begin{tabular}[c]{@{}c@{}}Embodiment\\ Error \%\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Reachability \\ Error \%\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Affordance\\ Errors \%\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Collisions\\ Per Episode\end{tabular}} \\ \midrule
% \rowcolor[HTML]{EFEFEF} 
% ReAct-Tools & Single & - & Oracle & Full & 0.88 & 5.40 & 1.25 & 0  \\
% ReAct-Tools & Multi & Centralized & Oracle & Full & 1.61 & 6.35 & 1.44 & 2  \\
% ReAct-Tools & Multi & Decentralized & Oracle & Full & 1.46 & 11.66 & 1.05 & 5 \\
% ReAct-Summary & Multi & Decentralized & Oracle & Full & 5.0 & 7.88 & 1.75 & 4  \\ \midrule
% \rowcolor[HTML]{EFEFEF} 
% ReAct-Tools & Single & - & Oracle & Partial & 1.79 & 3.90 & 1.01 & 0  \\
% ReAct-Tools & Multi & Decentralized & Oracle & Partial & 3.52 & 4.56 & 0.71 & 9  \\
% ReAct-Tools & Multi & Decentralized & Learned & Partial & 0.00 & 1.53 & 1.03 & 6  \\
% ReAct-Tools + RAG & Multi & Decentralized & Oracle & Partial & 1.87 & 4.49 & 0.69 & 8  \\
% ReAct-Summary & Multi & Decentralized & Oracle & Partial & 1.79 & 23.97 & 0.95 & 8  \\
% Finetuned-Summary & Multi & Decentralized & Oracle & Partial & 1.63 & 1.27 & 0.19 & 4  \\ \bottomrule
% \end{tabular}%
% }
% \vspace{3pt} 
% \caption{\textbf{Physical understanding errors.} We investigate embodiment errors, reachability errors, affordance errors and agent collisions. Each error cell indicates percent of low-level skills generated by the planner with respective errors averaged across all episodes for the robot agent.}
% \label{tab:physics}
% \end{table}



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % This table counts errors for ONLY robot
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{table}[h]
% % \begin{adjustbox}{width=\linewidth,center}
% % \centering
% % % \begin{table}[t]
% % % \centering
% % \small
% % \begin{tabular}{@{}ccccccccc@{}}
% % \toprule
% %          \textbf{Method}& \textbf{Agent}&  \makecell{\textbf{Perception} \\ \textbf{Tools}} & \textbf{Skills}& \textbf{Obs.}&  \makecell{\textbf{Embodiment} \\ \textbf{Error \(\%\)}}& \makecell{\textbf{Reachability} \\ \textbf{Error \(\%\)}}& \makecell{\textbf{Affordance} \\ \textbf{Errors \(\%\)}} & \makecell{\textbf{Collisions} \\ \textbf{per Episode}}\\
% % \midrule
% %          Centralized & Single& Yes& Oracle & Full & 0.88 & 5.40 & 1.25 & 0\\
% %          Centralized & Single& Yes& Oracle & Partial & 1.79 & 3.90 & 1.01 & 0\\
% %          Centralized & Multi& Yes& Oracle  & Full  & 1.61 & 6.35 & 1.44 & 2\\
% %          Decentralized & Multi& Yes& Oracle & Full & 1.46 & 11.66 & 1.05 & 5\\
% %          Decentralized & Multi& Yes& Oracle & Partial & 3.52 & 4.56 & 0.71 & 9\\
% %          Decentralized & Multi& Yes& Learned & Partial & 0.00 & 1.53 & 1.03 & 6\\
% %          Decentralized+RAG & Multi& Yes& Oracle & Partial & 1.87 & 4.49 & 0.69 & 8\\
% %          Decentralized & Multi& No & Oracle & Full & 5.0 & 7.88 & 1.75 & 4\\ 
% %          Decentralized & Multi& No & Oracle & Partial & 1.79 & 23.97 & 0.95 & 8\\
% %          Decentralized (FT) & Multi& No& Oracle & Partial & 1.63 & 1.27 & 0.19 & 4\\         
        
% % \bottomrule
% % \end{tabular}
% % % \end{table}
% % \end{adjustbox}
% % \vspace{3pt} 
% % \caption{Physical Error counts for different planner configurations, characterized by embodiment errors, reachability errors, affordance errors and agent collisions. Each error cell indicates percent of motor actions with respective errors averaged across all episodes for the robot agent.}
% % \label{tab:physics}
% % \end{table}

==> tables/task-division-analysis.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[htbp]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
\textbf{Method} & \textbf{Agent} & \textbf{Controllability} & \textbf{Skills} & \textbf{Observability} & \textbf{\begin{tabular}[c]{@{}c@{}}Robot\\ Moves\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Human\\ Moves\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Repeated\\ Moves\end{tabular}} \\ \midrule
ReAct-Tools & Multi & Centralized & Oracle & Full & 469 & 157 & 18 \\
ReAct-Tools & Multi & Decentralized & Oracle & Full & 521 & 512 & \textbf{189} \\
ReAct-Summary & Multi & Decentralized & Oracle & Full & 371 & 536 & 75 \\ \midrule
ReAct-Tools & Multi & Decentralized & Oracle & Partial & 494 & 399 & 118 \\
ReAct-Tools & Multi & Decentralized & Learned & Partial & 373 & 471 & 85 \\
ReAct-Tools + RAG & Multi & Decentralized & Oracle & Partial & 496 & 481 & 135 \\
ReAct-Summary & Multi & Decentralized & Oracle & Partial & 120 & 505 & 2 \todo{weird}\\
Finetuned-Summary & Multi & Decentralized & Oracle & Partial & 295 & 438 & 61 \\ \bottomrule
\end{tabular}%
}
\vspace{3pt} 
\caption{\textbf{Work distribution under different planner settings.} We measure the number of moves i.e., rearrangements, across human and robot, and the total number of moves repeated by both agents. Imbalanced workload highlighted by unequal moves across the agents and repeated rearrangements point to future avenues for improving collaborative planning.}
\label{tab:work-distribution}
\end{table}


% \begin{table}[h]
% %\begin{adjustbox}{width=\linewidth,center}
% \centering
% % \begin{table}[t]
% % \centering
% \small
% \begin{tabular}{@{}cccccccc@{}}
% \toprule
%          \textbf{Method}& \textbf{Agent}&  \makecell{\textbf{Perception} \\ \textbf{Tools}}& \textbf{Skills}& \textbf{Observability}&  \makecell{\textbf{Robot} \\ \textbf{Moves}}& \makecell{\textbf{Human} \\ \textbf{Moves}}& \makecell{\textbf{Repeated} \\ \textbf{moves}} \\
% \midrule
%          Centralized & Multi& Yes& Oracle  & Full  & 469 & 157 & 18 \\
%          Decentralized & Multi& Yes& Oracle & Full & 521 & 512 & 189 \\
%          Decentralized & Multi& Yes& Oracle & Partial & 494 & 399 & 118 \\
%          Decentralized & Multi& Yes& Learned & Partial & 373 & 471 & 85 \\
%          Decentralized+RAG & Multi& Yes& Oracle & Partial & 496 & 481 & 135 \\
%          Decentralized & Multi& No& Oracle & Full& 371 & 536 & 75  \\
%          Decentralized & Multi& No& Oracle & Partial& 120 & 505 & 2 \\
%          Decentralized (FT) & Multi& No& Oracle & Partial & 295 & 438 & 61\\           
% \bottomrule
% \end{tabular}
% % \end{table}
% %\end{adjustbox}
% \vspace{3pt} 
% \caption{Work distribution under different planner settings, categorized by number of robot moves, number of human moves, and the total number of moves repeated by both agents. Ideally the workload should be shared by both agents equally and there should be minimum number of repeated moves.}
% \label{tab:work-distribution}
% \end{table}

